Bounds on Sweep-Covers by Raney Numbers

In this work, we introduce a vertex separator in trees known as a sweep-cover that is defined by an ancestor-descendent relationship with all nodes in the tree. We prove the recurrence relation of sweep-covers with $n$ subcovers $P_{\Delta, \gamma}(n)$ on a class of infinite $\Delta$-ary trees with constant path lengths $\gamma$ between the $\Delta$-star internal nodes. Then, we provide recurrence relations for Raney numbers over integer compositions and show that they provide a lower-bound for sweep-covers such that $P_{\Delta, \gamma}(n) = \Omega\left( \frac{\sqrt{2 \pi} n^{\Delta n + \Delta + \frac{3}{2}}}{e^n ((\Delta-1)n+\Delta+1)!(n+1)!} \gamma \right)$.

==> Diagrams/LandRPartition.tex <==

\begin{figure}[!ht]
\begin{center}

\begin{tikzpicture}[scale = 0.23]

\def\nodesize{20pt}

    \node [circle, inner sep=0pt, minimum size=\nodesize, draw] (u) at (0,15)  {\footnotesize $v_s$};
    
    \node [circle, inner sep=0pt, minimum size=\nodesize, draw] (lu) at (0,10)  {\footnotesize $\mathcal{L}(v_s)$};
    
    \node [circle, inner sep=0pt, minimum size=17pt, draw] (c1) at (-10,0)  {\footnotesize $c_1$};
    
    \node [circle, inner sep=0pt, minimum size=17pt, draw] (c2) at (-5,0)  {\footnotesize $c_2$};
    
    \node [circle, inner sep=0pt, minimum size=17pt, draw] (c3) at (5,0)  {\footnotesize $c_3$};
    
    \node [circle, inner sep=0pt, minimum size=17pt, draw] (c4) at (8,0)  {\footnotesize $c_4$};
    
    
    \node [circle, inner sep=0pt, minimum size=17pt, draw] (c5) at (13,0)  {\footnotesize $c_5$};
    
    \node [circle, inner sep=0pt, minimum size=17pt, draw] (c6) at (16,0)  {\footnotesize $c_6$};
    \node [circle, inner sep=0pt, minimum size=17pt, draw] (c7) at (19,0)  {\footnotesize $c_7$};
    
    %Set Descriptors
    \node [ inner sep=0pt, minimum size=\nodesize] at (-12,0)  {\LARGE $\{$};
    
    \node [ inner sep=0pt, minimum size=\nodesize] at (-8,0)  {\LARGE $\}$};
    
    \node [ inner sep=0pt, minimum size=\nodesize] at (-7,0)  {\LARGE $\{$};
    
    \node [ inner sep=0pt, minimum size=\nodesize] at (-3,0)  {\LARGE $\}$};
    
    \node [ inner sep=0pt, minimum size=\nodesize] at (3,0)  {\LARGE $\{$};
    
    \node [ inner sep=0pt, minimum size=\nodesize] at (10,0)  {\LARGE $\}$};
    
    \node [ inner sep=0pt, minimum size=\nodesize] at (11,0)  {\LARGE $\{$};
    
    \node [ inner sep=0pt, minimum size=\nodesize] at (21,0)  {\LARGE $\}$};
    
    %L and R Descriptors
    \node [ inner sep=0pt, minimum size=\nodesize] at (10,-3)  {\LARGE $R$};
    
    \node [ inner sep=0pt, minimum size=\nodesize] at (-7,-3)  {\LARGE $L$};
    
 
%Define Edges
\draw [thick,dashed, ->] (u) -- node[above] {}  ++(lu);

\draw [thick, ->] (lu) -- node[above] {}  ++(c1);

\draw [thick, ->] (lu) -- node[above] {}  ++(c2);

\draw [thick, ->] (lu) -- node[above] {}  ++(c3);

\draw [thick, ->] (lu) -- node[above] {}  ++(c4);


\draw [thick, ->] (lu) -- node[above] {}  ++(c5);

\draw [thick, ->] (lu) -- node[above] {}  ++(c6);

\draw [thick, ->] (lu) -- node[above] {}  ++(c7);





  
\end{tikzpicture}
\caption{A partition of C into L and R where $C = \{ c_1, c_2, ... c_7\}$} \nopagebreak
\label{fig:LandRPartition}
 \nopagebreak
\end{center}
\end{figure}


==> Diagrams/Partition_Tree.tex <==

\begin{figure}[!ht]
\begin{center}

\begin{tikzpicture}[scale = 0.17]

\def\nodesize{17pt}

    \node [circle, inner sep=0pt, minimum size=\nodesize, draw] (a_1) at (0,20)  {\footnotesize $a_1$};
    
    \node [circle, inner sep=0pt, minimum size=\nodesize, draw] (a_2) at (0,14)  {\footnotesize $a_2$};

    \node [circle, inner sep=0pt, minimum size=\nodesize, draw] (a_c) at (0,5)  {\footnotesize $a_\gamma$};
    

    
      \node [circle, inner sep=0pt, minimum size=\nodesize, draw] (b_1) at (-6,3)  {\footnotesize $b_1$};

      \node [circle, inner sep=0pt, minimum size=\nodesize, draw] (d_1) at (6,3)  {\footnotesize $d_1$};
      
    \node [circle, inner sep=0pt, minimum size=\nodesize, draw] (c_1) at (0,0)  {\footnotesize $c_1$};

      \node [circle, inner sep=0pt, minimum size=\nodesize, draw] (b_c) at (-15,0)  {\footnotesize $b_\gamma$};
      
      \node [circle, inner sep=0pt, minimum size=\nodesize, draw] (c_c) at (0,-8)  {\footnotesize $c_\gamma$};
            
       \node [circle, inner sep=0pt, minimum size=\nodesize, draw] (d_c) at (15,0)  {\footnotesize $d_\gamma$};
       
     \node [circle, inner sep=0pt, minimum size=\nodesize, draw] (e_1) at (-22.5,0)  {\footnotesize $e_1$};
     
     \node [circle, inner sep=0pt, minimum size=\nodesize, draw] (f_1) at (-15,-7)  {\footnotesize $f_1$};
     
     \node [circle, inner sep=0pt, minimum size=\nodesize, draw] (g_1) at (-22.5,-7)  {\footnotesize $g_1$};
     
     \node [circle, inner sep=0pt, minimum size=\nodesize, draw] (h_1) at (-5,-15)  {\footnotesize $h_1$};
     
     \node [circle, inner sep=0pt, minimum size=\nodesize, draw] (i_1) at (0,-15)  {\footnotesize $i_1$};
     
     \node [circle, inner sep=0pt, minimum size=\nodesize, draw] (j_1) at (5,-15)  {\footnotesize $j_1$};
     
      \node [circle, inner sep=0pt, minimum size=\nodesize, draw] (k_1) at (22.5,0)  {\footnotesize $k_1$};
     
     \node [circle, inner sep=0pt, minimum size=\nodesize, draw] (l_1) at (15,-7)  {\footnotesize $l_1$};
     
     \node [circle, inner sep=0pt, minimum size=\nodesize, draw] (m_1) at (22.5,-7)  {\footnotesize $m_1$};
     
     
     
      
      
            
       
       
       
 
%Define Edges
\draw [thick, ->] (a_1) -- node[above] {\footnotesize $$}  ++(a_2);

\draw [thick, dashed, ->] (b_1) -- node[above] {\footnotesize $$}  ++(b_c);

\draw [thick, dashed, ->] (d_1) -- node[above] {\footnotesize $$}  ++(d_c);

\draw [thick, dashed, ->] (c_1) -- node[above] {\footnotesize $$}  ++(c_c);

\draw [thick, dashed, ->] (a_2) -- node[above] {\footnotesize $$}  ++(a_c);

\draw [thick, ->] (a_c) -- node[above] {\footnotesize $$}  ++(b_1);

\draw [thick, ->] (a_c) -- node[above] {\footnotesize $$}  ++(c_1);

\draw [thick, ->] (a_c) -- node[above] {\footnotesize $$}  ++(d_1);

\draw [thick, dashed, ->] (a_2) -- node[above] {\footnotesize $$}  ++(a_c);
\draw [thick, dashed, ->] (a_2) -- node[above] {\footnotesize $$}  ++(a_c);
\draw [thick, dashed, ->] (a_2) -- node[above] {\footnotesize $$}  ++(a_c);

%Define Edges
\draw [thick, ->] (b_c) -- node[above] {\footnotesize $$}  ++(e_1);
\draw [thick, ->] (b_c) -- node[above] {\footnotesize $$}  ++(f_1);
\draw [thick, ->] (b_c) -- node[above] {\footnotesize $$}  ++(g_1);

\draw [thick, ->](c_c) -- node[above] {\footnotesize $$}  ++(h_1);
\draw [thick, ->](c_c) -- node[above] {\footnotesize $$}  ++(i_1);
\draw [thick, ->](c_c) -- node[above] {\footnotesize $$}  ++(j_1);

\draw [thick, ->](d_c) -- node[above] {\footnotesize $$}  ++(k_1);
\draw [thick, ->](d_c) -- node[above] {\footnotesize $$}  ++(l_1);
\draw [thick, ->](d_c) -- node[above] {\footnotesize $$}  ++(m_1);


  
\end{tikzpicture}

\caption{$\mathcal{T}_{3,\gamma}$} \nopagebreak
\label{fig:Partition_Tree}
 \nopagebreak
\end{center}
\end{figure}


==> Diagrams/Sweep_Cover_Diagram.tex <==

\begin{figure}[!ht]
\begin{center}
\begin{comment}


\begin{tikzpicture}[scale = 0.25]

\def\nodesize{20pt}

    \node [circle, inner sep=0pt, minimum size=\nodesize, draw] (p) at (-5,10)  {\footnotesize $v_s$};

    \node [blue,circle, inner sep=0pt, minimum size=\nodesize, draw] (v) at (-10,5)  {\footnotesize $v_1$};
    
    \node [circle, inner sep=0pt, minimum size=\nodesize, draw] (u) at (0,5)  {\footnotesize $v_2$};
    
    \node [circle, inner sep=0pt, minimum size=\nodesize, draw] (Lu) at (0,0)  {\footnotesize $\mathcal{L}(v_2)$};
    
    \node [blue,circle, inner sep=0pt, minimum size=\nodesize, draw] (c1) at (-5,-5)  {\footnotesize $v_{c_1}$};
    
    \node [blue,circle, inner sep=0pt, minimum size=\nodesize, draw] (c2) at (0,-5)  {\footnotesize $v_{c_2}$};
    
    \node [blue,circle, inner sep=0pt, minimum size=\nodesize, draw] (c3) at (5,-5)  {\footnotesize $v_{c_3}$};
    
    \node [circle, inner sep=0pt, minimum size=\nodesize, draw] (d1) at (-5,-10)  {\footnotesize $v_{d_2}$};
    
    \node [circle, inner sep=0pt, minimum size=\nodesize, draw] (d2) at (-10,-10)  {\footnotesize $v_{d_1}$};
    
    %\node [circle, inner sep=0pt, minimum size=\nodesize, draw] (d3) at (5,-10)  {\footnotesize $d_3$};
    
    %Tikz is difficult so these are shoing the pursuer group travel paths
    
    \node (p11) at (-12.5,-7.5) {};
    
    \node (p21) at (-12.5,-7.5) {};
    
%Define Sweep Cover


%\draw  [rounded corners, dashdotted]   (-12, -12)  rectangle (-3, -8) {};

%\draw[rounded corners, dashdotted]  (7, -3)  rectangle  (-2, -7) {};
    
     
 
%Define Edges
%\draw [thick, ->] (u) -- node[above]   ++(u1) {};

\draw [thick, ->] (u) -- node[above]  {}  ++(Lu);
\draw [thick, ->] (Lu) -- node[above] {}  ++(c1);
\draw [thick, ->] (Lu) -- node[above] {} ++(c2);
\draw [thick, ->] (Lu) -- node[above] {} ++(c3);

\draw [thick, ->] (c1) -- node[above] {} ++(d1);
\draw [thick, ->] (c1) -- node[above] {} ++(d2);

\draw [thick,  ->] (p) -- node[above] {} ++(v);
\draw [thick,  ->] (p) -- node[above] {} ++(u);
%\draw [thick, ->] (c3) -- node[above]  ++(d3);

%Insert Legend

%\draw[]  (5,5)  rectangle  (15, 15) {};

  
\end{tikzpicture}

\end{comment}

\includegraphics[width=0.5\textwidth,keepaspectratio]{Diagrams/example_concepts.png}
\caption{Labeled tree with sweep cover $S = \{ \{ v_6 \},\{ v_4,v_5 \},\{ \mathcal{L}(v_2)\} \}$} \nopagebreak
\label{fig:Pursuer_Group_Sweep}
 \nopagebreak
\end{center}
\end{figure}


==> Diagrams/coral_diagram.tex <==

\begin{figure}[!ht]
\begin{center}

\begin{tikzpicture}[scale = 0.2]

\def\nodesize{17pt}


    \node [circle, inner sep=0pt, minimum size=\nodesize, draw] (s) at (0,5)  {\footnotesize $v_s$};
    
    \node [circle, inner sep=0pt, minimum size=\nodesize, draw] (v_1) at (-4,2)  {\footnotesize $v_1$};

    \node [circle, inner sep=0pt, minimum size=\nodesize, draw] (v_3) at (4,2)  {\footnotesize $v_3$};
    
    \node [circle, inner sep=0pt, minimum size=\nodesize, draw] (v_2) at (0,-2)  {\footnotesize $v_2$};
    
    
    \node [circle, inner sep=0pt, minimum size=\nodesize, draw] (b_1) at (10,2)  {\footnotesize $b_1$};

    \node [circle, inner sep=0pt, minimum size=\nodesize, draw] (b_2) at (10,-2)  {\footnotesize $b_2$};
    
    \node [circle, inner sep=0pt, minimum size=\nodesize, draw] (a_1) at (-10,2)  {\footnotesize $a_1$};

    \node [circle, inner sep=0pt, minimum size=\nodesize, draw] (a_2) at (-10,-2)  {\footnotesize $a_2$};
     
     
     
      
      
            
       
       
       
 
%Define Edges


\draw [thick,  ->] (s) -- node[above] {\footnotesize $$}  ++(v_1);


\draw [thick, ->] (s) -- node[above] {\footnotesize $$}  ++(v_2);
\draw [thick, ->] (s) -- node[above] {\footnotesize $$}  ++(v_3);


\draw [thick, ->] (v_3) -- node[above] {\footnotesize $$}  ++(b_1);
\draw [thick, ->] (v_3) -- node[above] {\footnotesize $$}  ++(b_2);

\draw [thick, ->] (v_1) -- node[above] {\footnotesize $$}  ++(a_1);
\draw [thick, ->] (v_1) -- node[above] {\footnotesize $$}  ++(a_2);






  
\end{tikzpicture}

\caption{A Raney Tree of (3,2,3) where the three internal nodes are $v_s$, $v_1$, and $v_2$} \nopagebreak
\label{fig:Raney_Tree}
 \nopagebreak
\end{center}
\end{figure}


==> Diagrams/embedding_tree_diagram.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{Diagrams/embedding_tree.png}
    \caption{Converting the sweep cover $S = \{ \{ v_4,v_5,v_6 \},\{ v_3 \} \}$ to an embedding tree defined by $\Upsilon_S=\{ v_5,v_3 \}$}
    \label{fig:embedding_tree}
\end{figure}

==> Text/Asymptotic.tex <==

\section{Asymptotic Bounds for Sweep-Covers}
\label{sec:Asymptotic_Analysis}

While the lower bounds proven in Section \ref{sec:Raney} are a nice connection to the Raney numbers, a lot of the structure is completely lost. Not to mention, we can show simpler lower bounds simply using the recurrence relation. 

\begin{lemma}
\begin{align}
    P_{\Delta,\gamma}(n) = \Omega(\Delta^{n-1})
\end{align}
\end{lemma}
\begin{proof}
Note that in (\ref{eq:Precurr_left}), for all $n>1$
\begin{align}
    P_{\Delta,\gamma}(n) &= \Delta\sum_{r=1}^{\Delta - 1} { L_{\Delta}(n-r,1) 
R(\Delta - 1,r)} + \ldots \\
&= \Delta P(n-1) + \ldots
\end{align}
\end{proof}

\subsection{Asymptotic Log-Convexity}
\begin{definition}[Asymptotic Log-Convexity]
We say a function $f(n)$ is asymptotically log-convex over an ordered domain if the function satisfies the following limit:
\begin{align}
    \lim_{n \rightarrow \infty} f(n)f(n-2) \geq f(n-1)^2. \label{eq:as_log_concavity}
\end{align}
If the inequality is strict then the function is considered strictly asymptotically log-convex. Note that a log-convex function satisfies the same relationship over an entire domain instead of with a limit.
\end{definition}

Note that in the limit of $n \rightarrow \infty$, asymptotically log-convex functions behave as if they are log-convex. So, the following proofs apply to asymptotically log-convex functions only as $n \rightarrow \infty$. The first useful property of log-convex functions is that their product over an integer partition is maximized when one input is maximized and the others are minimized. 

\begin{corollary}
Consider the log-convex function $f(n)$ over an ordered domain $\mathcal{C} \subseteq \mathbb{Z}_+$. Then, the following relationship holds for all $n$,
\begin{align}
   \forall n \in \mathcal{C} : \frac{f(a)}{f(a - 1)} \geq \ldots \geq  \frac{f(n)}{f(n-1)} \geq \frac{f(n-1)}{f(n-2)} \geq \ldots \geq  \frac{f(b + 1)}{f(b)},
\end{align}
where $a$ and $b$ are the supremum and infimum, respectively, of $\mathcal{C}$. \label{cor:log_convex_ratio}
\end{corollary}

\begin{lemma}
Consider a log-convex function $f$ over the ordered domain $\mathcal{C} \subseteq \mathbb{Z}_+$ with supremum $a$ and infimum $b$. Given any integer composition $X \in \Gamma_{n,m} \cap \mathcal{C}^m$, choose two parts in $x_j, x_v \in X$ such that $b < x_v \leq x_j < a$. Construct a new integer composition $\bar{X} = \{ \bar{x}_1,...,\bar{x}_{j}+1,...,\bar{x}_v-1,...,\bar{x}_m\}\}$. Then, the following relationship holds,
\begin{align}
    \prod_{x_k \in X}f(x_k) < \prod_{\bar{x}_k \in \bar{X}}f(\bar{x}_k). \label{eq:lem:log_convex_max_incr1}
\end{align}
\label{lem:log_convex_max}
\end{lemma}
\begin{proof}
By dividing both sides in (\ref{eq:lem:log_convex_max_incr1}) by all common factors and substituting in $\bar{x}_j = x_j + 1$ and $\bar{x}_v = x_v - 1$, we obtain
\begin{align}
    f(x_j)f(x_v) < f(x_j+1)f(x_v-1),
\end{align}
which is equivalent to Corollary \ref{cor:log_convex_ratio}.
\end{proof}

\begin{lemma}
By repeatedly applying Lemma \ref{lem:log_convex_max}, then the integer composition $X^* \in \Gamma_{n,m} \cap \mathcal{C}^m$ that maximizes the product $\prod_{x_k \in \bar{X}}f(x_k)$ is given by 
\begin{align}
    X^* = \begin{cases}\left\{ n - (m - 1)b, b, \ldots, b \right\} & \text{ for } n \leq a + (m - 1)b \\
    \{a\}^k\{\beta\}\{b\}^{m - k - 1} & \text{ for } n \geq a + (m - 1)b \text{ and }\beta > 0 \\ 
    \{a\}^k\{b\}^{m-k} & \text{ for } n \geq a + (m - 1)b \text{ and }\beta = 0
    \end{cases}.
    \label{eq:lem:log_convex_max_vector}
\end{align}
where $k \in \{1,\ldots,m\}$, $a$ and $b$ are the supremum and infimum of $\mathcal{C}$, and $\beta = n-kb \mod b$.
 \label{lem:log_convex_max_vector} 
\end{lemma}
\begin{proof}
If $n < mb$ or $n > ma$, then no integer composition exists where every part is in $\mathcal{C}$. Likewise, the maximum part in $X$ cannot exceed $a$ and the minimum cannot be below $b$. So, we can repeatedly apply Lemma \ref{lem:log_convex_max} on parts $x_j$ and $x_v$ until $x_j$ equals the maximum possible part, i.e., the minimum of $n - (m-1)b$ and $a$, or $x_v$ equals $b$. Then we consider a new pair and reapply Lemma \ref{lem:log_convex_max} until the same condition is met. We continue this process until all remaining parts are $b$. Note that $\beta$ occurs in a part when we cannot increase one part to $a$ but the remaining parts are all $a$ and $b$.
\end{proof}

\begin{lemma}
By repeatedly applying the inverse of Lemma \ref{lem:log_convex_max_vector}, the integer composition $\bar{X} \in \Gamma_{n,m} \cap \mathcal{C}^m$ that minimizes the product $\prod_{x_k \in X}f(x_k)$ when $f(n)$ is log-convex is any permutation of 
\begin{align}
    \bar{X} = \left\{\floor{\frac{n}{m}} + c_1, \floor{\frac{n}{m}} + c_2,  \ldots, \floor{\frac{n}{m}} + c_m \right\},
\end{align}
where $c_k \in \{0,1\}$ such that $\sum_{k \leq m}c_k < m$ and $b \leq \floor{\frac{n}{m}} \leq a$.\label{lem:log_concave_min_vector}
\end{lemma}
\begin{proof}
 Consider any integer composition $X \in \Gamma_{n,m} \cap \mathcal{C}^m$ and repeatedly apply the inverse of Lemma \ref{lem:log_convex_max} to reduce the product $\prod_{x_k \in \bar{X}}f(x_k)$. The final integer composition will be a permutation of $\bar{X}$. 
\end{proof}

\subsection{Upper-Bounds on Sweep-Covers}

To begin probing the asymptotics of the recurrence relation, we first consider (\ref{eq:Precurr_mid}). Note that the number of integer compositions of $n$ into $m$ parts is log-convex, therefore, the leading asymptotic of $P_{\Delta,\gamma}(n)$ is likely also log-convex. Also note that by having a leading asymptotic that is log-convex, it does not imply the function is log-convex in the same region as the leading asymptotic. Because the recurrence relation is consistent for all $n \geq \Delta$, it's easy to show by contradiction that the leading asymptotic term in $P_{\Delta,\gamma}(n)$ is the same term for all $n \geq \Delta$. So, we assume the leading asymptotic of $P_{\Delta,\gamma}(n)$ is log-convex with respect to $n$ for all $n$. Assuming log-convexity, we can upper-bound $L_\Delta(n,m)$ by the integer composition $X^*$ that maximizes the product in Lemma \ref{lem:log_convex_max_vector}. Therefore, by enumerating all integer compositions, the following bound always holds,
\begin{align}
    L_\Delta(n,m) < &\binom{n - 1}{m - 1}P_{\Delta,\gamma}(n - b(m - 1))P_{\Delta,\gamma}(b)^{m-1}. \label{eq:L_convex_ub}
\end{align}
By the same argument, if the leading asymptotic of $P_{\Delta,\gamma}(n)$ is log-convex in the region $n \geq \Delta$, then the infimum $b$ must be less than $\Delta$. By a similar contradiction proof in the region $n < \Delta$, $R(\Delta,m)$ does not grow faster than any other term. So, the leading asymptotic in the region $n < \Delta$, is given by some $r$ and $l$ in (\ref{eq:Precurr_left}). However, the upper bounds on the summation in (\ref{eq:Precurr_left}) can be rewritten as
\begin{align}
    P_{\Delta,\gamma}(n) &= \sum_{l=1}^{n-2}\binom{\Delta}{l}\sum_{r=1}^{n-l}L_\Delta(n-r,l)R(\Delta-l,r) + R(\Delta,n).
\end{align}

Therefore, eventually the leading asymptotic given by the worst case $r$ and $l$ will not be a term in for all $n < \Delta$. For simplicity, we will assume the leading asymptotic in the region $n < \Delta$ is the same as in $n \geq \Delta$.


One can already loosely see the leading log-convex asymptotic. By applying the upper bound in (\ref{eq:L_convex_ub}) to the recurrence relation, we can keep pulling out terms of the form $(n - b_1(m_1-1))^{m_1-1}(n - b_2(m_2-1))^{m_2-1}...(n - b_\mu(m_\mu-1))^{m_\mu-1}$. The depth of this recurrence is on the order of $n / \sum_i b_i(m_i-1)$ which gives a log-convex asymptotic on the order of the Pochhammer symbol. 








Next, we assume log-convexity for the leading term in the asymptotic of $P_{\Delta,\gamma}(n)$. This does not imply that $P_{\Delta,\gamma}(n)$ itself is always log-convex.
Next, note that any part $x_j \in X^*$ is upper bounded by $n - m + 1$. So, if we assume the upper bound (\ref{eq:L_ub}) for each $L_\Delta$ term in the summation in $P_{\Delta,\gamma}(n - m + 1)$, we can pull out $n - 2m + 2$ so we have 

\begin{align}
    L_\Delta(n,m) < \left(\frac{n - 1}{m - 1}\right)^{m-1}\prod_{x_j \in X^*}P_{\Delta,\gamma}(x_j). \label{eq:L_ub}
\end{align}

by lower bounding each part by $P_{\Delta,\gamma}(x_j) > L_\Delta(x_j,m_j)$ we obtain, 

\begin{align}
    P_{\Delta,\gamma}(n) = O\left(2^{\Delta n}(\Delta \gamma)^{n-1}\left(\frac{n - 1}{\Delta - 1}\right)^{(n)}\right)
\end{align}

\begin{align}
    \sum_{l=1}^{n-2}\binom{\Delta}{l} = (2^\Delta - 2\Delta - 1)
\end{align}


\begin{align}
    P_{\Delta,\gamma}(n) < 2^{\Delta n}(\Delta \gamma)^{n-1}b^b\prod_{k_1=1}^{h_1}(n-k_1(r+b(l-1)))
\end{align}
where $b < \Delta$.
We justify this ansatz by noting the relationship 

For $n > \Delta$,
\begin{align}
    P_{\Delta,\gamma}(n) &= \sum_{l=1}^{\Delta-2}\binom{\Delta}{l}\sum_{r=1}^{\Delta-l}L_\Delta(n-r,l)R(\Delta-l,r)  + L_\Delta(n,\Delta) \\
\end{align}
To begin we approximate an upper bound on the summation by assuming the worst case parameterization of $l$, i.e., $l'$ across the entire sum. Additionally, to avoid an undefined asymptotic when we expand $L_\Delta(n-r,1)$, we separate $l=1$ from the outer sum. So, we are left with,
\begin{align}
    P_{\Delta,\gamma}(n) < & (2^\Delta - 2\Delta - 1)\sum_{r=1}^{\Delta-l'}L_\Delta(n-r,l')R(\Delta-l',r)  + L_\Delta(n,\Delta) \\&+ \sum_{r=1}^{\Delta - 1}\Delta P(n-1) R(\Delta - 1,r).
\end{align}
We can expand $L_\Delta(n,m)$ into an asymptotic by assuming the worst-case integer composition that maximizes the ansatz,
\begin{align}
    L_\Delta(n,m) < &\binom{n - 1}{m - 1}P_{\Delta,\gamma}(n - b(m - 1))P_{\Delta,\gamma}(b)^{m-1} \\
    < & \left(\frac{(n-1)}{(m-1)}\right)^{m-1} 2^{\Delta n}(\Delta \gamma)^{n - l} P_{\Delta,\gamma}(n - b(m - 1)) P_{\Delta,\gamma}(b)^{m-1}.
\end{align}
As we will see shortly, this assumption does not degrade the upper bound too much considering the exponential terms in the ansatz add across the product to the same term for nearly all integer compositions, except when $b = 1$. 





\begin{lemma}
\begin{align}
    P_{\Delta,\gamma}(n) = \Omega((\gamma+1)^{n-1})
\end{align}
\end{lemma}
\begin{proof}
For any $2 \leq n < \Delta$, there always exists a term $(P_{\Delta,\gamma}(1))^{n-1}$ in (\ref{eq:Precurr_left}) when $l = n-1$ and $r=1$. For $n \geq \Delta$, there always exists a term in (\ref{eq:Precurr_mid}) such that $P_{\Delta,\gamma}(n-\Delta+1)(P_{\Delta,\gamma}(1))^{\Delta-1} = \Omega((\gamma+1)^{n-1})$.
\end{proof}

\begin{lemma}
    There exists a fixed term in $P_{\Delta,\gamma}(n)$ with the greatest asymptotic complexity for all $n$.
\end{lemma}

In this section, we prove Theorem \ref{thm:P_n_tight} by using log-convexity properties of the asymptotic expansion of $P_{\Delta,\gamma}(n)$.
\begin{theorem}
\begin{align}
    P_{\Delta,\gamma}(n) = \Theta_{\Delta,\gamma}(n^{n+1})
\end{align}
\label{thm:P_n_tight}
\end{theorem}



\subsection{Tight Bounds for Increasing Subcovers}
Here, we will prove Theorem \ref{thm:P_n_tight} by induction using an ansatz of $P_{\Delta,\gamma}(n) = \Theta(n^{n+1})$. First, we rewrite $P_{\Delta,\gamma}(n)$ as an asymptotic expansion such that the first term satisfies the ansatz,
\begin{align}
    P_{\Delta,\gamma}(n) = \Theta(n^{n+1}) + \sum_{i=1}^N c_i f_i(n), \label{eq:P_asymptotic_expansion}
\end{align}
where $c_i$ and $f_i(n)$ are constants and functions, respectively, that approximate $P_{\Delta,\gamma}(n)$. Here, $f_i(n) = o(f_{i-1}(n))$ so no function grows faster than $f_0(n) = \Theta(n^{n+1})$. However, $P_{\Delta,\gamma}(n)$ must also grow at least as fast as $f_0(n)$. So, we split the ansatz expansion into two expansions and prove both by induction,
\begin{align}
    P_{\Delta,\gamma}(n) = O(n^{n+1}) + \sum_{i=1}^N c_i f_i(n) \label{eq:P_ansatz_ub}\\
    P_{\Delta,\gamma}(n) = \Omega(n^{n+1}) + \sum_{i=1}^N c_i f_i(n). \label{eq:P_ansatz_lb}
\end{align}

\begin{lemma}
\begin{align}
P_{\Delta,\gamma}(n) = O(n^{n+1}) \label{eq:P_n_ub}
\end{align}
\label{lem:P_n_ub}
\end{lemma}
\begin{proof}
The base case is satisfied for $n=1$. For the inductive step, consider the fact that $\Delta$ and $\gamma$ are constant and much smaller than $n$. Then, $P_{\Delta,\gamma}(n)$ is a summation over $L_\Delta(n-r,l)$ with constant coefficients. Therefore, we only need to show that $L_\Delta(n-r,l) = O(n^{n+1})$ is true for all $r$ and $l$. Substituting the ansatz (\ref{eq:P_ansatz_ub}) into (\ref{eq:LDelta}) yields
\begin{align}
L_\Delta(n-r,l) = \sum_{X \in \Gamma_{n-r,l} }{\prod_{x_j \in X}[O(x_j^{x_j+1}) + \sum_{i=1}^N c_i f_i(x_j)]}.
\end{align}
Expanding the product and using $f_i(n) = o(f_0(n))$ implies
\begin{align}
    \prod_{x_j \in X}[O(x_j^{x_j+1}) + \sum_{i=1}^N c_i f_i(x_j)] = O(\prod_{x_j \in X}x_j^{x_j+1}) + o(\prod_{x_j \in X}x_j^{x_j+1}). \label{eq:lem:P_ub:prod_ub}
\end{align}
We drop the right term in (\ref{eq:lem:P_ub:prod_ub}) because it cannot grow faster than the left term. One can verify that the ansatz in (\ref{eq:P_n_ub}) is asymptotically log-convex. Therefore, the integer composition $\bar{X} \in \Gamma_{n-r,l}$ that maximizes $\prod_{x_j \in X}x_j^{x_j+1}$ is given by Lemma \ref{lem:log_convex_max_vector}. If we assume every integer composition is replaced by the upper-bound $\bar{X}$, then (\ref{eq:lem:P_ub:prod_ub}) becomes
\begin{align}
L_\Delta(n,1) = & \Omega\left(\binom{n - r - 1}{l - 1}\left( n - r - l + 1 \right)^{n - r - l + 2}|_{r=0,l=1}\right) \nonumber \\ 
= & \Omega\left( n^{n+1}\right)
\label{eq:lem:P_lb:prod_ub2}
\end{align}
 To obtain the asymptotic maximum, we approximate $\binom{n - r - 1}{l - 1}$ using the well-known upper bound of $\binom{n - r - 1}{l - 1} < \frac{(n - r - 1)^{l-1}}{(l-1)!}$. Because $r$ and $l$ are bounded constants, reducing them to maximize $\frac{n - r}{l}$ will maximize the order of (\ref{eq:lem:P_ub:prod_ub2}), i.e., setting $r = 0$ and $l = 1$ implies $\beta = 0$. This reduces (\ref{eq:lem:P_ub:prod_ub2}) to
\begin{align}
    L_\Delta(n,1) = O(n^{n+1}).
\end{align}
\end{proof}

\begin{lemma}
\begin{align}
P_{\Delta,\gamma}(n) = \Omega(n^{n+1}) \label{eq:P_n_lb}
\end{align}
\label{lem:P_n_lb}
\end{lemma}
\begin{proof}
Applying similar arguments as in Lemma \ref{lem:P_n_ub}, we can express the asymptotic lower-bound of $P_{\Delta,\gamma}(n)$ as the lower-bound of the fastest growing term $L_\Delta(n-r,l)$ when $r = 0$, $l = 1$. By applying the ansatz (\ref{eq:P_ansatz_lb}), along with Lemma \ref{lem:log_concave_min_vector}, we can rewrite $L_\Delta(n-r,l)$ as
\begin{align}
L_\Delta(n-r,l) =  &O\left(\beta \binom{n - r - 1}{l - 1}\left( \frac{n - r}{l } + 1 \right)^{\frac{n - r}{l} + 2}\right) \nonumber\\
+ &O\left((l - \beta)\binom{n - r - 1}{l - 1}\left( \frac{n - r}{l} \right)^{\frac{n - r}{l} + 1}\right), \label{eq:lem:P_ub:prod_ub2}
\end{align}

where $\beta = n - r \mod l$.
\end{proof}
Then, Theorem \ref{thm:P_n_tight} follows from Lemmas \ref{lem:P_n_ub} and \ref{lem:P_n_lb}.



==> Text/Term_Glossary.tex <==
Directed Tree - $\mathcal{T}$
Nodes in Tree - $\mathcal{V}$
Edges in Tree - $\mathcal{E}$
Sweep-Cover   - $S$
Root Node     - $v_s$
Leaf Nodes    - $\mathcal{G}$


==> Text/convexity_dump.tex <==

\begin{lemma}
  $L_\Delta(n,\Delta)$ is log-convex for $n > \Delta$.
\end{lemma}
\begin{proof}
To show $L_\Delta(n,\Delta)$ is log-convex, we will use induction. Consider the base-case of $n = \Delta + 2$ and the associated inequality,
\begin{align}
    \frac{L_\Delta(\Delta + 2,\Delta)}{L_\Delta(\Delta + 1,\Delta)} > \frac{L_\Delta(\Delta + 1,\Delta)}{L_\Delta(\Delta,\Delta)}.
\end{align}
Using Definition \ref{def:Ldelta}, the inequality becomes
\begin{align}
    \frac{L_\Delta(\Delta + 2,\Delta)}{L_\Delta(\Delta + 1,\Delta)} > \frac{L_\Delta(\Delta + 1,\Delta)}{L_\Delta(\Delta,\Delta)}.
\end{align}
\end{proof}

\begin{lemma}
  $L_\Delta(n,m)$ is log-convex for $n > m$ and constant $m$.
\end{lemma}
\begin{proof}
To show $L_\Delta(n,m)$ is log-convex, we will use induction. First, consider the fact that for $n < m$ and $m > \Delta$, $L_\Delta(n,m) = 0$. Then, the base case must be for $n = m + 2$ for any $0 < m \leq \Delta$. Hence, consider some constant $m \in (0,\Delta]$ for the following inequality:
\begin{align}
    \frac{L_\Delta(m + 2,m)}{L_\Delta(m + 1,m)} > \frac{L_\Delta(m + 1,m)}{L_\Delta(m,m)}.
\end{align}

\begin{align}
    \frac{{m \choose 2} P(2) P(2) P(1)^{m-2} + m P(3) P(1)^{m - 1}}{m P(2) P(1)^{m-1}} > \frac{m P(2)}{P(1)}.
\end{align}
Which implies the following true inequality,
\begin{align}
    \frac{{m \choose 2} P(2) }{m P(1)} + \frac{P(3)}{P(2)} > \frac{m P(2)}{P(1)}.
\end{align}

Now, consider any $n > m + 2$. Assume the inductive step, 

\begin{align}
    \frac{L_\Delta(n,m)}{L_\Delta(n-1,m)} > \frac{L_\Delta(n-1,m)}{L_\Delta(n-2,m)} > ... > \frac{L_\Delta(m + 1,m)}{L_\Delta(m,m)}.
\end{align}

Now, we will prove that 

\begin{align}
  L_\Delta(n+1,m)L_\Delta(n-1,m) > L_\Delta(n,m)L_\Delta(n,m). \label{eq:lem:P_log_convex1}
\end{align}



First, consider the fact that we can decompose $L_\Delta(n+1,m)$ into summations over $\Gamma_{n-1,m}$, $\Gamma_{n-1,m - 1}$, and $\Gamma_{n-1,m - 2}$, i.e.,
\begin{align}
    L_\Delta(n+1,m)  = & \sum_{X \in \Gamma_{n+1,m}}\prod_{x_j \in X}P_{\Delta,\gamma}(x_j) \nonumber \\ = & \sum_{X \in \Gamma_{n,m}}\sum_{i = 1}^m P_{\Delta,\gamma}(x_i + 1 )\prod_{x_j \in X \backslash x_i }P_{\Delta,\gamma}(x_j) + mP(1)L_{\Delta}(n,m-1) \label{eq:lem:P_log_convex2} \\  = & \sum_{X \in \Gamma_{n-1,m}}\sum_{i = 1}^m P_{\Delta,\gamma}(x_i + 1 )\sum_{j = 1, j \ne i}^m P_{\Delta,\gamma}(x_j + 1 )\prod_{x_k \in X \backslash x_i,x_j }P_{\Delta,\gamma}(x_k) \label{eq:lem:P_log_convex3.1} \\ & + \sum_{X \in \Gamma_{n-1,m}}\sum_{i = 1}^m P_{\Delta,\gamma}(x_i + 2 )\prod_{x_k \in X \backslash x_i }P_{\Delta,\gamma}(x_k) \label{eq:lem:P_log_convex3.2} \\ & + mP(2)L_{\Delta}(n-1,m-1) \label{eq:lem:P_log_convex3.3} \\ & + {m \choose 2}P(1)^2L_{\Delta}(n-1,m-2). \label{eq:lem:P_log_convex3.4}
\end{align}

Likewise, we can obtain a similar identity for $L_\Delta(n,m)$ over $\Gamma_{n-1,m}$ and $\Gamma_{n-1,m - 1}$,

\begin{align}
    L_\Delta(n,m)  = \sum_{X \in \Gamma_{n-1,m}}\sum_{i = 1}^m P_{\Delta,\gamma}(x_i + 1 )\prod_{x_j \in X \backslash x_i }P_{\Delta,\gamma}(x_j) + mP(1)L_{\Delta}(n-1,m-1) \label{eq:lem:P_log_convex4}
\end{align}

Then, by applying 

\end{proof}

\begin{theorem}
Consider a positive, monotonically increasing function $f(x)$ over $[0,\infty)$ such that:
\begin{align}
    &\forall x \in [0,\infty) : f'(x) \geq 0 \\
    &\forall x \in [0,\infty) : f''(x) > 0 \\ 
    &\forall x \in [0,\infty) : f''(x)f(x) > (f'(x))^2
\end{align}

 Let $h(x)$ be an asymptotic upper bound on $f(x)$ such that $f(x) = \Theta(h(x))$. Define $g(n,i)$ to be a summation of the products of $f$ over integer compositions of $n$ into $i$ parts. 

\begin{equation}
    g(n,i) = \sum_{X \in \Gamma_{n,i} }{(\prod_{x_j \in X}f(x_j))} 
\end{equation}
Then, $g(n,i) = \Theta(h(n-1)^{n-1}h(1)^{i-1})$.
\label{thm:int_comp_convex_func}
\end{theorem}
We will prove Theorem \ref{thm:int_comp_convex_func} using the following proofs.

\begin{definition}[Convex Set]
The set $S$ is considered a convex set if the line between every pair of points $x,y \in S$ is also contained in $S$. Namely, let $\theta \in [0,1]$, then $\forall \theta : \theta x + (1 - \theta)y \in S$. 
\label{def:convex_set}
\end{definition}

We will consider the following set to be the domain of interest for analysis of the convex function $f(x)$. 

\begin{lemma}
The set $Y_{n,p} \subset \mathbb{R}^p$ that contains all points which satisfy the following inequality is convex.
\begin{equation}
    y_1 + y_2 + ... + y_p \leq n
\end{equation}
\begin{equation}
    \forall y_i \in y : y_i > 1
\end{equation}
\label{lem:polytope_convexity}
\end{lemma}
\begin{proof}
Applying Definition \ref{def:convex_set}, consider any two points $x,y \in Y$. Then, $\forall x,y \in Y : \theta x + (1 - \theta) y \in Y$. This implies that the sum of all components for $x$ and $y$, when multiplied by their new coefficients, should also satisfy the inequality. 

\begin{equation}
    z = \theta x + (1 - \theta) y
\end{equation}

\begin{equation}
    z_1 + z_2 + ... + z_p = \theta \sum_{x_j \in x} x_j + (1 - \theta)\sum_{y_j \in y} y_j \leq \theta n + (1 - \theta) n
\end{equation}

Additionally, consider $z_i = \theta x_i + (1 - \theta) y_i$. If both $x_i > 1$ and $y_i > 1$ then $z_i > 1$. Which implies that $\forall \theta : z = \theta x + (1 - \theta) y \in Y$ so $Y$ is a convex set.
\end{proof}

The convex polytope that satisfies the following inequality $x_1 + x_2 + ... x_p \leq n$ contains all integer partitions of $n$ into $p$ parts. Using analysis of convex functions, it is easy to show that the upper bound on a product of monotonic, increasing log-convex functions $Y$ is the point where $x_1 = x_2 = ... x_p = n/p$ which is a valid integer partition for all $n \in \mathbb{Z}_+$ divisible by $p$. 

\begin{definition}[Convex Function]
Consider a function $f$ and a convex set $Y$. We say $f$ is convex if $\forall x,y \in Y$, the following inequality holds.

\begin{equation}
    \forall x,y \in Y : \theta f(x) + (1 - \theta)f(y) \leq f(\theta x + (1 - \theta)y)
\end{equation}
\end{definition}

\begin{definition}[Log-Convex Function]
Consider a function $f$ and a convex set $Y$. We say $f$ is log-convex if $\forall x,y \in Y$, the following inequality holds.
\begin{equation}
    \forall x,y \in Y : \theta \log f(x) + (1 - \theta) \log f(y) \leq \log f(\theta x + (1 - \theta)y)
\end{equation}
One can easily show that log-convexity is equivalent to the following if $f(x)$ is twice differentiable:
\begin{equation}
    \forall x,y \in Y : f''(x)f(x) > (f'(x))^2
\end{equation}
\end{definition}

\begin{lemma}
Let $g : \mathbb{R}^p \rightarrow \mathbb{R}$ be the product of a log-convex function $f : \mathbb{R} \rightarrow \mathbb{R}$ over the components of $\mathbf{x}$ where $\mathbf{x}$ is an element of the convex polytope $Y_{n,p}$. 

\begin{equation}
    g(\mathbf{x}) = {\prod_{x_j \in \mathbf{x}}f(x_j)} 
\end{equation}
Then, $g(\mathbf{x})$ is a convex function over $Y_{n,p}$.
\label{lem:product_log_convexity}
\end{lemma}
\begin{proof}
  By Lemma \ref{lem:polytope_convexity}, the convex polytope $Y_{n,p}$ is a convex set.
  Define a family of functions $F = \{f_1,f_2,...,f_i\}$ such that $f_j(\mathbf{x}) = f(x_j)$. Then, $g(\mathbf{x})$ is isomorphic to the product across the family of functions over the same vector $\mathbb{x} \in Y_{n,p}$. To show this product is convex, we rely on the fact that the log-convexity of a function implies the function is also convex. 
 \begin{equation}
     \log(\prod_{j = 1}^pf_j(\mathbf{x})) = \sum_{j = 1}^p\log f_j(\mathbf{x}) \cong \sum_{x_j \in \mathbf{x}}\log f(x_j) 
 \end{equation}
 The log of the product becomes a sum of convex functions because $log f$ is convex by definition. Then, the product across $F$ is log-convex, which implies it is also convex. 
\end{proof}

\begin{lemma}
Let $g : \mathbb{R}^p \rightarrow \mathbb{R}$ be the product of a non-decreasing, log-convex function $f : \mathbb{R} \rightarrow \mathbb{R}$ over the components of $\mathbf{x}$ where $\mathbf{x}$ is an element of the convex polytope $Y_{n,p}$. 

\begin{equation}
    g(\mathbf{x}) = {\prod_{x_j \in \mathbf{x}}f(x_j)} 
\end{equation}
Then, the vector which maximizes $g$ is given by $\mathbf{x}' = \{ \frac{n}{p},  \frac{n}{p}, ...,  \frac{n}{p} \}$.
\end{lemma}
\begin{proof}
 First, note that the components of the maximum vector $\mathbf{x}'$ must sum to $n$ because $f$ is non-decreasing. So, we can reparameterize the problem over a 
 
 By Lemma \ref{lem:product_log_convexity}, $g$ is convex. Then, the maximum of a convex function is wherever the 
\end{proof}


\subsection{Log-Convexity of Enumerating Sweep-Covers}

To show the asymptotic relation for $P_{\Delta,\gamma}(n)$, we will prove a more general recurrence relation and show that $P_{\Delta,\gamma}(n)$ is a special case.

If upper bounds for $L_{\Delta}(n,m)$ and $R(n,m)$ are known for any given $n$ and $m$, then we can show an upper bound on $P_{\Delta,\gamma}(n)$. However, showing an upper bound for $L_{\Delta}(n,m)$ is a subtle process. Arguments from convexity require that the function be continuous. But, enumerative functions are usually discrete. To remedy this, consider the function $\tilde{P}_{\Delta,\gamma}(n)$ to be a smooth continuous function, twice differentiable everywhere such that $\forall n \in \mathbf{Z}^+ : \tilde{P}_{\Delta,\gamma}(n) = P_{\Delta,\gamma}(n)$.

It is quite easy to show that if $P_{\Delta,\gamma}(n)$ 

The first useful property is that the second-order and first order forward difference of $P_{\Delta,\gamma}(n)$ is always positive. For notational brevity, we will drop the subscripts $\Delta,\gamma$ on $P_{\Delta,\gamma}(n)$ and $\tilde{P}_{\Delta,\gamma}(n)$, but their dependence is implied throughout the following proofs.

\begin{lemma}[First-Order Forward Difference]
$\forall n > 0, \forall h > 0 : $ 
\begin{equation}
    \frac{P(n+h) - P(n) }{h} > 0
\end{equation}
\label{lem:first_order_fwd_difference}
\end{lemma}
\begin{proof}
 It suffices to show that $P(n)$ is monotonic increasing, i.e., $\forall n > 0 : P(n+1) - P(n) > 0$. Then, by induction the above inequality will hold for all $h$, i.e., $P(n+h) > P(n + h - 1) > P(n + h - 2) > ... > P(n) \implies P(n+h) - P(n) > 0 \implies \frac{P(n+h) - P(n) }{h} > 0$. By Corollary \ref{cor:generating_function}, the partition $X$ of $n-1$ such that $X = \{n-1\}$ is considered in the generating function for all $n$. One can easily verify that every other term in the summation is strictly positive by definition. So,  $P(n) = \Delta R(\Delta-1,1)P(n-1) + ... > P(n-1)$. 
\end{proof}

\begin{lemma}[Second-Order Forward Difference]
$\forall n,h > 0$
\begin{equation}
    \frac{P(n+2h) - 2P(n+h) + P(n) }{h^2} > 0
\end{equation}
\end{lemma}
\begin{proof}
 It suffices to show that $\forall n,h > 0 : P(n+2h) > 2P(n+h)$. Using a similar proof to Lemma \ref{lem:first_order_fwd_difference}, $P(n) = \Delta R(\Delta-1,1)P(n-1) + ... > \Delta P(n-1) \implies P(n + 2h) > \Delta P(n + 2h - 1) ... > \Delta^h P(n + h) > 2P(n+h)$. 
\end{proof}

\begin{lemma}
The average rate of change in the second derivative of $\tilde{P}_{\Delta,\gamma}(n)$ is positive for all $n > 0$.
\end{lemma}
\begin{proof}
 
\end{proof}



\begin{lemma}
Consider a monotonic, increasing function $P$ whose logarithm is convex, i.e. $\log P(y)$. Then, the following product is a convex function for all points in 

\begin{equation}
    \forall y \in Y : \prod_{y_j \in y}P(y_j)
\end{equation}
\end{lemma}
\begin{proof}
 
 \begin{equation}
 \theta \prod_{x_j \in x}P(x_j) + (1 - \theta)\prod_{y_j \in y}P(y_j) \leq \prod_{x_j,y_j \in x,y}P(\theta x + (1 - \theta)y)
 \end{equation}
 
 $\forall x,y > 1 : \log(x + y) < \log(x) + \log(y)$, then $\log x + \log y \leq \log z$
 
\end{proof}



==> Text/embedding_trees.tex <==

\subsection{Embedding Trees}
\begin{definition}[Embedding Trees from Sweep-Covers]
Given a tree $\mathcal{T} = \{\mathcal{V}, \mathcal{E} \}$ and a sweep-cover $S$, let $\Upsilon_S$ be a set containing one node from each subcover in $S$. Define $\mathcal{V}_S$ and $\mathcal{E}_S$ to be the union of all nodes and edges, respectively, of all paths from the source node in $\mathcal{T}$ to each node in $\Upsilon_S$. Then, the tree $\mathcal{T}_S = \{\mathcal{V}_S \subseteq \mathcal{V}, \mathcal{E}_S \subseteq \mathcal{E} \}$ is an embedding tree for the sweep-cover $S$ on $\mathcal{T}$.
\end{definition}

\input{Diagrams/embedding_tree_diagram}

%\begin{corollary}
%A countably infinite set of distinctly labeled sweep-covers corresponds to any given embedding tree if the maximum out degree of the original tree is infinite. 
% \label{cor:infinite_sweep_covers}
%\end{corollary}
%\begin{proof}
%An embedding tree is created by selecting a single node from a set of sibling nodes. That set of sibling nodes can have a cardinality of any size so the number of possible sweep-covers that could create that embedding tree is infinite.
%\end{proof}

\begin{corollary}
The set of all possible embedding trees on any tree is equal to the set of all finite trees.
 \label{cor:all_trees_are_embedding}
\end{corollary}
\begin{proof}
 $\mathcal{T} = \{ \mathcal{V}, \mathcal{E}\}$. 
Given any finite tree $\mathcal{T} = \{ \mathcal{V}, \mathcal{E}\}$, let $\mathcal{G} \subset \mathcal{V}$ be the set of all leaf nodes in a $\mathcal{T}$. The collection $S = \{ \forall g \in \mathcal{G} : \{g\} \}$ containing a singleton of each leaf node is a valid sweep-cover whose embedding tree is isomorphic to $\mathcal{T}$. The embedding tree for this sweep-cover is isomorphic to $\mathcal{T}$. Conversely, every embedding tree constructed from a sweep-cover is a finite tree.
\end{proof}

\begin{lemma}
 All embedding trees created from the same sweep-cover are isomorphic.
 \label{lem:isomorphic_embedding_trees}
\end{lemma}
\begin{proof}
 This is provable by contradiction. For a given embedding tree, it has an associated set $\Upsilon_S$ which is defined by taking a single node from each subcover in S. All possible embedding trees defined by the same $\Upsilon_S$ are isomorphic. So, $\Upsilon_S$ must differ for two heteromorphic embedding trees. Let's denote the different sets to be $\Upsilon_S$ and $\Upsilon'_S$, each constructed from S. By definition of a sweep-cover, each set in S must be composed of sibling nodes. Therefore, for any given node in which $\Upsilon_S$ and $\Upsilon'_S$ differ, one of its sibling nodes must exist in the other set. So, there exists a bijection from $\Upsilon_S$ and $\Upsilon'_S$ by membership in a set in S. Likewise, there also exists a bijection by the edges defined from their parent node. Finally, because the same paths go from the source node to the parent node of every set of siblings, the differences in each embedding tree exist only between the differing sibling nodes and the related edges from the shared parent node. However, there exists a bijection between these differences. Therefore, there exists a bijection between both trees and they are isomorphic. 
\end{proof}

\begin{lemma}
    Denote the set of all  sweep-covers with n subcovers to be $\mathcal{M}$ and the set of all heteromorphic n-leaf trees to be  $\mathcal{N}$. Construct a mapping $\mathcal{H}: M \rightarrow N$ by taking every sweep-cover $S \in \mathcal{M}$ and map it to an n-leaf tree $\mathcal{T} \in \mathcal{N}$ such that $\mathcal{T}$ is isomorphic to the embedding tree created by $S$. 
    
    Then,  $\mathcal{H}$ is surjective, non-injective, and every sweep-cover maps to one heteromorphic embedding tree.
     \label{lem:surjective_mapping}
\end{lemma}

\begin{proof}
By Corollary \ref{cor:all_trees_are_embedding}, there always exists a sweep-cover of size $n$ for a given n-leaf tree. So the mapping is surjective. Also, due to the definition of the leaf nodes by $\Upsilon_s$, the number of leaves in an embedding tree is equal to the number of sets in the corresponding sweep-cover so all n-leaf embedding trees map from some sweep-cover of size n. Consider a sweep-cover which contains a partition of a set of sibling nodes into at least 2 sets, each of which contains more than 1 node. Construct a second sweep-cover by picking 1 node from each of 2 sets of the partitioned sibling nodes and placing them in the other set. Define their corresponding $\Upsilon_S$ sets by selecting any of the unswapped nodes. Their embedding trees will be isomorphic but the sweep-covers will differ. Therefore, two different sweep-covers can create the same embedding tree so the mapping is non-injective.
 
 Because all embedding trees created from a sweep-cover are isomorphic by Lemma \ref{lem:isomorphic_embedding_trees}, and all trees in the co-domain are heteromorphic with respect to all the other trees in the co-domain, the sweep-cover will map to an embedding tree which is isomorphic to one and only one tree in the co-domain.
\end{proof}




%\begin{theorem}
%There does not exist a bijective mapping from Raney trees with n-leaf nodes to sweep-covers of size n.  \label{lemma:inverse_mapping_lemma}
%\end{theorem}
%\begin{proof}
%Because all n-leaf embedding trees are mapped to by at least one sweep-cover of size n by Corollary \ref{cor:surjective_mapping} and there exists embedding trees which are not isomorphic to Raney trees by Corollary \ref{cor:Embedding_not_Raney} and there cannot exist two 
%\end{proof}

%\subsection{sweep-cover - Raney Conjecture}
%Lemma \ref{cor:Embedding_not_Raney} presents a 

%illustrate the difficulty of connecting Raney trees with sweep-covers and why a more general description of trees is required. Due to Corollary \ref{cor:Embedding_not_Raney}, enumerating all possible sweep-covers which correspond to a given embedding tree cannot provide a connection to Raney trees. Therefore, a more generalized description of trees is required. However, 
\begin{comment}


\begin{definition}
Consider the class of all heteromorphic trees which can be constructed by $n$ internal nodes, of which any internal node may have an out-degree $\leq \Delta$. Denote this class of trees to be $\Phi$-trees. Let the enumeration of all $\Phi$-trees for a given $\Delta$ and n internal nodes be $\Phi_\Delta(n)$
\end{definition}

\begin{lemma}
The enumeration of all $\Phi$-trees with n internal nodes and a p-star root such that all children are internal nodes is the following expression assuming $\Phi_\Delta(k_j)$ is defined for all $k_j < n$.
\begin{equation}
    \sum_{K \in \mathcal{U}^{n-1}_p} \prod_{k_j \in K} \Phi_\Delta(k_j)
\end{equation}
\label{lem:Phi_internal_recurrence}
\end{lemma}

\begin{proof}
Consider an integer partition $K$ into $p$ parts which is an element of $\mathcal{U}^{n-1}_p$ as in Definition \ref{def:unordered_integer_parts}. For each part $k_j \in K$, construct a $\Phi$-tree of $k_j$ internal nodes. Then, define a p-star as a root node and let the root node for each $\Phi$-tree be a child of the p-star. This $\Phi$-tree contains $n$ internal nodes. One can see that this $\Phi$-tree is also inherently heteromorphic to all other $\Phi$-trees defined by different integer partitions of $n-1$ into $p$ parts because the expression only considers unordered integer partitions, which are all unique and exhaustive of $n$. However, ordered integer partitions are isomorphic by commuting terms in the product.

%Therefore, the enumeration of all ways of constructing $\Phi$-trees in this manner, i.e. considering all possible p-star roots, all $l \leq p$, and all integer partitions of $K$ into $l$ parts, is the same as the recurrence relation above. 
\end{proof}


\begin{lemma}
A recursive expression which enumerates all $\Phi$-trees of a given $\Delta$ and $n$ is the following:
\begin{equation}
    \Phi_\Delta(1) = \Delta
\end{equation}
\begin{equation}
    \Phi_\Delta(n) = \sum_{p = 1}^{\Delta} \sum_{l = 1}^{p} \sum_{K \in \mathcal{U}^{n-1}_l} \prod_{k_j \in K} \Phi_\Delta(k_j)
\end{equation}
\label{lem:recurrence_of_Phi}
\end{lemma}

\begin{proof}
Proof by induction. Naturally, the base case is just all possible p-stars of which there are $\Delta$. Then, assuming the expression is correct for $n - 1$ and some $\Delta$, I must prove that all $\Phi$-trees of $n$ and $\Delta$ can be constructed from $\Phi$-trees of $n-1$ and $\Delta$. First, consider all possible p-stars as the root node. These are all heteromorphic with respect to each other and it is exhaustive of all possible roots of the tree. Then, all heteromorphic trees of n internal nodes of a given p-star as the root can be constructed by considering all ways of constructing the $n-1$ internal nodes from descendants of the root. All ways of doing this can be enumerated by considering all $l \leq p$ of the children of the p-star and constructing the tree from these $l$ children where each of these children will be an internal node and therefore contributing to the internal node count. However, the other $p - l$ children will not contribute to the internal node count but they are still considered in the enumeration because they are inherently heteromorphic. So, the number of heteromorphic trees with an l-star root is the same as the number of heteromorphic trees with a p-star root where only l children are internal nodes. By Lemma \ref{lem:Phi_internal_recurrence} the enumeration of all $\Phi$-trees with $n$ internal nodes and an l-star root is given by the inner product and summation. This expression is then exhaustive.

%To prove that these are the only heteromorphic trees can be done by contradiction. Suppose there existed a $\Phi$-tree constructed without this manner. By definition, the root must have out-degree $\leq \Delta$ 
 
\end{proof}



\begin{definition}
Consider the class of all labeled trees which can be constructed by $n$ internal nodes, of which any internal node may have an out-degree $\leq \Delta$. Denote this class of trees to be $\Omega$-trees. Let the enumeration of all $\Omega$-trees for a given $\Delta$ and n internal nodes be $\Phi_\Delta(n)$
\end{definition}

\begin{lemma}
The enumeration of all $\Phi$-trees with n internal nodes and a p-star root such that all children of the p-star are internal nodes is:
\begin{equation}
    \sum_{K \in \mathcal{O}^{n-1}_p} \prod_{k_j \in K} \Phi_\Delta(k_j)
\end{equation}
\label{lem:Omega_internal_recurrence}
\end{lemma}

\begin{proof}
If all children of the p-star are internal nodes, then for each internal node consider that the root of some new $\Phi$-tree with some integer number of internal nodes. To consider all possible ways of constructing a tree from the children of the p-star, take an integer partition of $K$ into $p$ parts, which is an element of $\mathcal{O}^{n-1}_p$ as in Definition \ref{def:ordered_integer_parts}. For each part $k_j \in K$, construct a $\Phi$-tree of $k_j$ internal nodes. Then, define a p-star as a root node and let the root node for each $\Phi$-tree be a child of the p-star. This $\Phi$-tree contains $n$ internal nodes. 

%This is proven by the same argument in Lemma \ref{lem:Phi_internal_recurrence} except labels are not commutative so the ordering of the integer partition matters. Therefore, the sum is taken with respect to all ordered integer partitions.
\end{proof}


\begin{lemma}
A recursive expression which enumerates all $\Phi$-trees of a given $\Delta$ and $n$ internal nodes is the following:
\begin{equation}
    \Phi_\Delta(1) = \Delta
\end{equation}
\begin{equation}
    \Phi_\Delta(n) = \sum_{p = 1}^{\Delta} \sum_{l = 1}^{p} { p \choose l } \sum_{K \in \mathcal{O}^{n-1}_l} \prod_{k_j \in K} \Phi_\Delta(k_j)
    \label{eq:omega_enum}
\end{equation}
\label{lem:recurrence_of_Omega}
\end{lemma}

\begin{proof}
Proof by induction. Naturally, the base case is just all possible p-stars of which there are $\Delta$. Then, assume the expression is correct for $n - 1$ and some $\Delta$. First, consider all possible p-stars from $p=1$ to $p=\Delta$ as the root node. These are all heteromorphic with respect to each other and it is exhaustive of all possible roots of the tree. Then, all heteromorphic trees of n internal nodes of a given p-star as the root can be constructed by considering all ways of constructing the $n-1$ internal nodes from descendants of the root. Some internal nodes must come from the children of the root, and which children are chosen can be enumerated by ${p \choose l}$ for all $l \leq p$. Given $l$ children which will contribute to the internal node count, Lemma \ref{lem:Omega_internal_recurrence} provides the recursive enumeration of all $\Phi$-trees rooted at the $l$ children.
 
\end{proof}
\end{comment}


==> Text/removed_asymptotics.tex <==

\subsection{Asymptotic Upper Bound of Enumerating Constant Sized Sweep-Covers With Respect to the Maximum Out Degree, $\Delta$}
Here our inductive step is slightly different from what one might expect. Because $P_{\Delta,\gamma}(n)$ is recursive with respect to $n$ and not $\Delta$, we have to be careful about our inductive step. In simple terms, we are interested in how the number of sweep-covers scales with $\Delta$. If our inductive step is analyzed with respect to $P_{\Delta,\gamma}(n)$, it is very difficult to account for all changes in out-degree of the structure at once and write down one term to express this. So, we have to consider the asymptotic ratio downstream. If we assume an asymptotic of $P_{n,\gamma}(\Delta) = f(\Delta)$, then for any recursive instance of $P_{\Delta,\gamma}(n)$, assume that all the out-degrees downstream have been increased by one. If the inductive step holds that we see the same ratio increase in this ratio, then the asymptotic is preserved overall. Assume c is some unknown constant. If $n$ and $\gamma$ are constant, then:
\begin{lemma}
 \begin{equation}
     P_{n,\gamma}(\Delta) = O(\Delta^{c}c^\Delta)
 \end{equation}
\end{lemma}
\begin{proof}
First, it's important to note that for $\Delta >> n$, $l \leq n - 1$ and $r < n - l$, otherwise $L_{\Delta}(n-r,l) = 0$. This implies the summation bounds can be relaxed to 
\begin{equation}
    P_{\Delta,\gamma}(n) = \sum_{l=1}^{n - 1}{ \binom{\Delta} {l}  \sum_{r=1}^{n - l} {L_{\Delta}(n-r,l)R(\Delta - l,r)}}.
\end{equation}
By definition, $R(\Delta - l,r) <  \stirling{\Delta - l}{r} < \frac{r^\Delta}{r!} $ by assuming $r$ is fixed. Using induction, assume $P_{\Delta,\gamma}(n) = O(\Delta^{c}c^\Delta)$ and naturally the base case is satisfied if $\gamma$ is constant. Then, $L_{\Delta,\gamma}(n-r,l) < n^lc^{l\Delta}\Delta^{cl}$ which implies 
\begin{equation}
    P_{\Delta,\gamma}(n) < \sum_{l=1}^{n}{ \binom{\Delta} {l}  \sum_{r=1}^{n - 1} {n^lc_2^{l\Delta}\Delta^{c_1l}\frac{r^\Delta}{r!}}} + \frac{n^\Delta}{n!}
\end{equation}
Note that $L_{\Delta,\gamma}(n,\Delta) = 0$ for $\Delta > n$ and $R(\Delta,n) < \frac{n^\Delta}{n!}$. Relax the inner boundary by assuming $r = c_3$ and multiplying by $n$. This is permissible because r is upper bounded by the constant n and we'll see that so long as r is any constant, the inequality will hold.

\begin{equation}
    P_{\Delta,\gamma}(n) < \sum_{l=1}^{n}{ \binom{\Delta} {l}  \Delta^{c_1l}n^{l+1}\frac{c_2^{l\Delta}c_3^\Delta}{c_3!}} + \frac{n^\Delta}{n!}
\end{equation}

Likewise, for any fixed $l$ and increasing $\Delta$, $\binom{\Delta}{l} = \frac{\Delta!}{l! (\Delta - l)!}$, therefore:

\begin{equation}
    P_{\Delta,\gamma}(n) < \sum_{l=1}^{n}{ \frac{\Delta!}{l! (\Delta - l)!}  \Delta^{c_1l}n^{l+1}\frac{c_2^{(l + 1)\Delta}}{c_3!}} + \frac{n^\Delta}{n!}
\end{equation}

Relax the boundary further by assuming any worst case constant for l and multiplying by $n$. This is permissible because the upper boundary on l is the constant n. Then, take the infinite limit with respect to $\Delta$
\begin{equation}
    P_{\Delta,\gamma}(n) < \lim_{\Delta \rightarrow \infty}{ \frac{\Delta!}{l! (\Delta - l)!}  \Delta^{c_1l} n^{l+2}\frac{c_2^{l \Delta }c_3^\Delta}{c_3!}} + \frac{n^\Delta}{n!}
\end{equation}

Then, simplify constants. 

\begin{equation}
    P_{\Delta,\gamma}(n) < \lim_{\Delta \rightarrow \infty}{ \frac{\Delta!}{l! (\Delta - l)!}  \Delta^{c}\frac{c^{l \Delta }c^\Delta}{c!}} + \frac{c^\Delta}{c!}
\end{equation}
Using $\frac{\Delta!}{(\Delta - l)!} = \prod_{i = 0}^{l-1}{(\Delta - i)} < \Delta^l$
\begin{equation}
    < \lim_{\Delta \rightarrow \infty}{ \Delta^l  \Delta^{c}\frac{c^{l \Delta }c^\Delta}{c!}} + \frac{c^\Delta}{c!} = O(c^\Delta \Delta^c)
\end{equation}

\end{proof}

\subsection{Asymptotic Upper Bound of Enumerating Constant Sized Sweep-Covers With Respect to Linear Path Length, $\gamma$}

\begin{lemma}
  \begin{equation}
     P_{\Delta,\gamma}(n) = O(\gamma^n)
 \end{equation}
\end{lemma}

\begin{proof}
Assuming $\Delta$ and $n$ are constant, and $\Delta < n$, then $R(\cdot,\cdot)$ is constant. By induction, assume the relation holds for smaller $\gamma$.
\begin{equation}
    L_{\Delta,\gamma}(n,i) = \sum_{K \in \mathcal{O}^n_i}{(\prod_{k_j \in K}P_{\Delta,\gamma}( k_j ))}
\end{equation}

\begin{equation}
    = \sum_{K \in \mathcal{O}^n_i}{O(\gamma^n)}
\end{equation}
For fixed n and i,
\begin{equation}
    = {O(\gamma^{n})}
\end{equation}

Then,
    
\begin{equation}
    P_{\Delta,\gamma}(n) = \sum_{l=1}^{n}{ \binom{\Delta} {l}  \sum_{r=1}^{n - 1} {O(\gamma^{l(n-r)}})} + O(\gamma^n)
\end{equation}

%\begin{equation}
%    = \sum_{l=1}^{n}{ \binom{\Delta} {l}  \sum_{r=1}^{n - l} {O(\gamma^{l(n-r)}})} + O(\gamma^n)
%\end{equation}

\begin{equation}
    =  O(\gamma^n)
\end{equation}

\end{proof}

==> Text/scrap_definitions.tex <==

\begin{definition} [Depth]
Let $\mathcal{T}= \{\mathcal{V}, \mathcal{E}\}$ be a directed tree, with a root node, $v_s \in \mathcal{V}$.  Define the {\it depth} of a given node $v \in \mathcal{V}$, to be the number of edges in the unique path from $v_s$ to $v$ in the tree. Assume that the depth of the source node $v_s$ is 0.
\label{def:depth}
\end{definition}

\begin{definition} [Linear Path]
We define a linear path $L \subset \mathcal{E}$ to be an ordered set of edges $L = \{ (v_{i_1}, v_{i_2}), (v_{i_2},v_{i_3})  ... (v_{i_{m-1}},v_{i_m}) \}$ that connects the initial node $v_{i_1}$ to the terminal node $v_{i_m}$ such that each edge's source node along the linear path has at most one outgoing edge in $\mathcal{E}$.
\label{def:Linear_Path}
\end{definition}

\begin{definition}[Lowest Known Descendant]
For each node $v \in \mathcal{V}$, define $\mathcal{L}(v)$ to be the descendant of $v$ (or $v$ itself) such that a linear path exists from  $v$ to $\mathcal{L}(v)$ and $\mathcal{L}(v)$ has an out degree not equal to 1 \cite{Sundaram2016PursuitEvasion}. 
\label{def:lowest_known_descendant}
\end{definition}

==> Text/scrap_lemmas.tex <==

\begin{lemma}
All possible sweep-covers $S$ on a tree $\mathcal{T}$ where $|S| > 1$ can be found by Lemma \ref{lem:swap_children} or Lemma \ref{lem:singleton}. \label{lem:all_sweep_covers}
\end{lemma}
\begin{proof}
This can be proven by contradiction. Suppose there to be a sweep cover, $S$, of size $n > 1$ which cannot be defined by Lemma \ref{lem:singleton} or a partition of $C$, denoted as $C'$. There are 3 potential sets for the nodes in $S$: $\mathcal{A}_{C'}$, $\mathcal{D}_{C'}$ or $C'$. If a set in $S$ is in $\mathcal{A}_{C'}$, then $S$ must be a sweep cover of size 1, otherwise $S$ violates Definition \ref{def:SweepCover}.\ref{sweep_cover:ancestor}. $S$ cannot be a partition of $C$, otherwise $S$ is defined by Lemma \ref{lem:swap_children}. If $S$ contains a subset of $C$, the other sets in $S$ must be descendants of the other nodes, in C to avoid being a partition of $C$, as they can't be ancestors or they violate Definition \ref{def:SweepCover}.\ref{sweep_cover:ancestor}. Therefore, if $S$ exists then a sub-collection of its sets,  $S' \subseteq S$, must contain nodes in $\mathcal{D}_{C'}$ but not be defined by Lemma \ref{lem:singleton}. This implies that any subset of $S'$ cannot be a sweep cover of a subtree, $\mathcal{T}'$, rooted by any of the nodes in $C$ because this is defined by Lemma \ref{lem:singleton}. However, if $S'$ cannot form a sweep cover of $\mathcal{T}'$ then it can't be for violating Definitions \ref{def:SweepCover}.\ref{sweep_cover:disjointne}, \ref{def:SweepCover}.\ref{sweep_cover:sibling}, or \ref{def:SweepCover}.\ref{sweep_cover:ancestor} because these violations cannot be fixed by adding the remaining sets in $S$. So, $S'$ must violate Definition \ref{def:SweepCover}.\ref{sweep_cover:complete_graph}. Therefore, there exist nodes in $\mathcal{T}'$ which are not in $S'$ or an ancestor or descendant of $S'$ however they are a descendant of the root of $\mathcal{T}'$. Because the remaining nodes in S cannot be an ancestor of any nodes in $\mathcal{T}'$, otherwise they would violate Definition \ref{def:SweepCover}.\ref{sweep_cover:ancestor} with a node in $S'$, the descendant relationship of a node in S cannot fix a violation of Definition \ref{def:SweepCover}.\ref{sweep_cover:complete_graph} by S'. Therefore, S also violates Definition \ref{def:SweepCover}.\ref{sweep_cover:complete_graph} and is not a sweep cover. 

%Therefore, the sets in $S$ must be in $\mathcal{D}_C$ which implies $C$ is a subset of the ancestors of $\cup S$ and $S$ must each create sweep covers of the subtrees rooted by $c$.
%Consider a partition of $C$ in to $|C|$ parts and an application of Lemma \ref{lem:singleton} on this partition. Then, any sweep cover, $S$, produced by this method is composed of nodes in $c \cup \mathcal{D}_c$ and each subtree rooted by a node in $c$ must have a sweep-cover in $S$.  Then, $S$ is equivalent to $S$ and can be defined by Lemma \ref{lem:singleton}. 



%and apply the same argument, then we can see that if $P$ contains any parts of $c$ or is strictly contained in $\mathcal{D}_c$ (in the case of the partition of $c$ into $|c|$ parts), then Lemma \ref{lem:singleton} can define the partition. Therefore, $P$ can only be defined by Lemma \ref{lem:singleton}.


%Therefore, any subtree rooted by a node in $c$ which also has a sweep-cover in $P$ has no nodes in $P'$. Also, no sets in $P'$ are in the subtree. Otherwise, the nodes in the set would be in the descendants or ancestors of the sweep-cover in $P$ which violates subdefinition \ref{sweep_cover:ancestor} of a sweep-cover. Consequently, the sets in $P'$ must be in some subtree rooted by nodes in $C$ which do not have a sweep-cover in $P$. However, if these sets do not form a sweep-cover of the subtree, then one of the subdefinitions does not hold for the sets in $P'$. subdefinitions \ref{sweep_cover:disjointne}, \ref{sweep_cover:sibling}, and \ref{sweep_cover:ancestor} of a sweep cover must hold for any subset of sets in $P$. However, subdefinition \ref{sweep_cover:complete_graph} can only be true when considering all nodes in $P$. Therefore, the sets in $P'$ must hold all subdefinitions except subdefinition \ref{sweep_cover:complete_graph} for $P$ to be considered a sweep-cover and the sets in $P'$ to not be considered sweep covers for any subtree rooted by a node in $c$. If this is the case, then there exist some nodes which are not in $\mathcal{A}_{P'} \cup \mathcal{D}_{P'} \cup P' = \mathcal{V'}$ but are in the same subtree as some nodes in $P'$. These nodes cannot have an ancestor in $P$ because then that ancestor would also be an ancestor to some nodes in $P'$ which violates subdefinition \ref{sweep_cover:ancestor}. There also cannot exist a descendant to these nodes in $P$ because then they would form a sweep-cover with the sets in $P'$. Therefore, these nodes are not in $\mathcal{V'}$ and consequently cannot satisfy subdefinition \ref{sweep_cover:complete_graph}. So $P$ cannot be considered a sweep-cover.
\end{proof}

\begin{lemma}
Consider any tree $\mathcal{T}$ and a sweep-cover $S$. Let $\mathcal{P}_S$ be the set of all parents of the nodes in $S$. Define another sweep-cover $S'$ by replacing the necessary sets of nodes in $S$ with new sets of nodes taken from $\mathcal{P}_S$. Then, $|S'| \leq |S|$ where $|S|$ is the number of sets of nodes in $S$.
 \label{cor:ancestors_smaller_sweep_covers}
\end{lemma}
\begin{proof}
 This follows directly from the fact that Lemma \ref{lem:swap_children} can only maintain or increase the number of subcovers. However, Corollary \ref{cor:sc_partition_parent_construction} can only decrease the number of subcovers because the in-degree of every node is one. To see this, choose a subset of nodes $P \subseteq \mathcal{P}_S$. All subcovers that are descendants of 
\end{proof}
\begin{proof}
We will prove this by contradiction. Assume that 

For the base case, consider a sweep-cover $S$ that contains a singleton for every leaf node in the tree. Let $\mathcal{P}$ be the set of all the parents of the nodes in $S$. Because the in-degree of every leaf node is one, every singleton in $S$ has only one parent. Likewise, for each node $v_p$ in $\mathcal{P}$, $S$ contains a partition of the children of $v_p$. So, 

only the source node $v_s \in \mathcal{T}$. There are no ancestors for $v_s$, so $\mathcal{A}_{S} = \emptyset$. If $S' = \{\{\emptyset\}\}$, then $|S'| \leq |S|$. Now, consider any sweep-cover $S$ for a tree $\mathcal{}$


Suppose that $|S'| > |S|$. Then, for each set $S_z$ in $S$, there exists at least one set $S'_x$ in $S'$ that contains nodes which are ancestors of the nodes in $S_z$. Because the in-degree is always one in trees and all sets in a sweep-cover are siblings, if a node in $S'_x$ is an ancestor of one node in $S_z$, it is an ancestor of all nodes in $S_z$. 

However, if $|S'| > |S|$, then there also exist additional sets which must also be ancestors of the nodes in $S$. So, 

Then, by a counting argument, $S'$ contains at least two sets $S'_x$ and $S'_y$ that share descendants contained in one subcover in $S$, e.g., $S_z \in S$.

If $S'$ is a sweep-cover, then $S'_x$ and $S'_y$ cannot be an ancestor or descendant of one another. In order for this to be the case, and for both of them to contain ancestors of $S_z$, they must be subsets of two distinct sets of ancestors that converge at a given node, i.e., there must exist two nodes, $v_i \in \mathcal{A}_{S_z}$ and $v_j \in \mathcal{A}_{S_z}$ such that $S'_x \subset \mathcal{A}_{\{v_i\}} \wedge S'_y \nsubset \mathcal{A}_{\{v_i\}}$ and $S'_y \subset \mathcal{A}_{\{v_j\}} \wedge S'_x \nsubset \mathcal{A}_{\{v_j\}}$. However, this implies the existence of a third node $v_h$ such that $S'_x \cup S'_y \in \mathcal{A}_{v_h}$ which is only true if $v_h$ has two incoming edges. But, then $v_h$ violates the definition of a tree with two incoming edges.


%whose nodes are some ancestors of the nodes in $S$. However, they cannot be ancestors of any nodes in $S'$ otherwise Definition \ref{def:SweepCover}.\ref{sweep_cover:ancestor} is violated. So, each node in $S_x$ must be an ancestor of a set $S_y \in S - S' \cap S$, i.e., $S_x \subset \mathcal{A}_{S_y}$. By definition of a tree, there cannot exist multiple incoming edges to a node in a tree. If $S'_x$ contains multiple nodes, they must be sibling nodes. However, because a node cannot have multiple incoming edges in a tree, the sibling nodes in $S'_x$ will have unique descendants, i.e. $\forall v_i, v_j \in S'_x : \mathcal{D}_{v_i} \cap \mathcal{D}_{v_j} = \emptyset$. By Definition \ref{def:SweepCover}.\ref{sweep_cover:complete_graph}, if $S_y \subset \mathcal{D}_{v_j}$, then there exists some node $v_i \in S'_x$ and some subcover $S_z \in S$ such that $S_z \subset \mathcal{D}_{v_i}$, otherwise either $S$ or $S'$ are not sweep-covers. If this is the case, then $S_z \nin S'$ so $|S'| = |S - S_y - S_z \cup S'_x| < |S|$. If $S'_x$ is a singleton with multiple children, then $S_y$ must be a subset of descendants of one child and $S_z$ will be a subset of descendants of another child. So, the same argument can be applied. Finally, if $S'_x$ is a singleton such that there exists a linear path between $v \in S'_x$ and the parent of the nodes in $S_y$, then $S = $

%For any other case, define a subset of subcovers $\bar{S} \subset S$. Then, construct a collection of nodes $\bar{A}$ by choosing from the ancestors of the nodes in $\bar{S}$, i.e., $\bar{A} = \{ \bar{A}_j \in \bar{A} :  A_j \subset \bigcup_{S_i \in \bar{S}}\mathcal{A}_{S_i} \}$. Define a new collection $S' = S \backslash S_i \cup  \bar{A} $. Now, replace a set of nodes, $S_i \in S'$, with a singleton of one their ancestor nodes, $v_a \in \mathcal{A}_{S_i}$. For every other subcover whose ancestor is $v_a$, we must remove it from $S$ when constructing $S'$. Otherwise, $S'$ violates Definition \ref{def:SweepCover}.\ref{sweep_cover:ancestor}. If $v_a$ is an ancestor to 


%Applying Lemma \ref{lem:swap_children}, any ancestor of a node in a subcover $S_i$ will be an ancestor to all of the 


%the same ancestors and descendants of $S_i$ because all nodes in $S_i$ are siblings. If $v_a$ is only an ancestor of the nodes in $S_i$, then $|S'| = |S|$. However, if $v_a$ is also an ancestor of other nodes in $S'$, or if we selected $v_a$'s siblings, there are descendants of $S_i'$ in $S'$, and they must be removed from $S'$. Therefore, $|S'| \leq |S|$.
\end{proof}


\begin{corollary}
Consider a tree $\mathcal{T}$ with $n$ leaf nodes, then the maximum size of a sweep-cover S on $\mathcal{T}$ is $n$.
\end{corollary}
\begin{proof}
 Let S be a collection of singletons of the leaf nodes. Trivially, this collection is a sweep-cover, and it is the maximum sized sweep-cover which can be constructed from the leaf nodes. By Lemma \ref{lem:ancestors_smaller_sweep_covers}, any sweep-covers constructed from ancestors of $S$ must have a smaller size than $S$. Because there are no descendants of the leaf nodes, we cannot create greater sized sweep-covers from their descendants. Therefore, S is the largest sweep-cover which can be constructed from the leaf nodes and the maximum sized sweep-cover on $\mathcal{T}$.
\end{proof}


\begin{lemma}
Consider a partition of $C$, $p(C)$. Define $L \subseteq C'$  to be the collection of singletons in $C'$ and $R \subseteq C'$ to be the collection of non-singleton sets in $C'$, i.e. $C'\backslash L$. For each singleton $L_i \in L$, construct a subtree $T_i$ by taking all descendants of $c_i \in L_i$, and their associated edges in $\mathcal{T}$. Construct a collection of sets $Z = \{ Z_1, Z_2, ..., Z_{|L|}\}$ by taking a sweep-cover $Z_i$ from every subtree $T_i$. Then, the collection $S' = Z \cup R$ is a valid sweep-cover.
\label{lem:singleton}
\end{lemma}
\begin{proof}

\begin{figure}
    \centering
    \includegraphics[width=0.7\textwidth]{Diagrams/LR_Diagram.png}
\caption{A partition of C into L and R where $C = \{ c_1, c_2, ... c_7\}$} 
\label{fig:LandRPartition}

\end{figure}

%\input{Diagrams/LandRPartition.tex}

If $|L| = 0$, then by Lemma \ref{lem:swap_children}, $R$ is a sweep cover. Because the descendants of every node in $C$ are distinct, each sweep-cover will be distinct and disjoint so the collection $S'$ will be disjoint, thereby satisfying Definition \ref{def:SweepCover}.\ref{sweep_cover:disjointne}. Every pairwise set of nodes in $R$ and every subcover in every sweep-cover in $Z$ only contain sibling nodes. So, $S'$ only contains sibling nodes in each set and satisfies Definition \ref{def:SweepCover}.\ref{sweep_cover:sibling}. Because $\mathcal{V}_i = \mathcal{D}_{\{c_i\}} \cup c_i$, one can easily verify that $\bigcup_{c_i \in L} \mathcal{V}_i \cup R \cup \mathcal{A}_{\cup_{S_i \in R}} \cup \mathcal{D}_{\cup_{S_i \in R}}$ which satisfies Definition \ref{def:SweepCover}.\ref{sweep_cover:complete_graph}. Finally, because each sweep-cover is constructed from non-overlapping subtrees, they cannot be ancestors or descendants of one another. Likewise, because each sweep-cover in $Z$ comes from a subtree rooted by a sibling node to each node in $R$, they cannot be ancestors or descendants of any node in $R$. Therefore, $S'$ satisfies Definition \ref{def:SweepCover}.\ref{sweep_cover:ancestor} and is a sweep-cover.

%Because its sweep-cover $Z_i$ will be disjoint from every other sweep-cover $Z_j$ and $R$ because the descendants of every node in $C$ are distinct, i.e., $\forall c_i, c_j \in C : \mathcal{D}_{}$. 





%fill the remaining $n - |R|$ sets, find all ways of appending sweep covers from the subtrees rooted by the singletons in $L$ to construct larger sweep covers whose size is $n$. Each singleton contributes a single sweep cover such that the total sets of nodes in the sweep-covers sum to $n - |R|$.

%In order to achieve this, consider an ordered partition of the integer $n - |R|$ into each singleton in $l_i \in L$. Each part is the size of a sweep-cover required from the $l_i$ singleton's subtree. To find all possible ways of applying this method to a given partition of C, consider all ordered partitions of the integer $n - |R|$ into $L$ parts. For each ordered partition, find all of the sweep covers on a given subtree for its assigned integer part size. For a given ordered integer partition, consider all sweep covers which can be created by initializing the collection $R$ and then appending exactly one sweep cover (size defined by integer part) from each subtree. This will create all sweep covers of size $n = |R| + (n - |R|)$ which can be defined by this method.
\end{proof}



\begin{theorem}
Algorithm \ref{alg:Find_Sweep_Covers} returns all sweep covers of size $n$ from $\mathcal{T}$. If none are possible, then the algorithm returns an empty set.
\label{thm:correctness:full_correctness}
\end{theorem}

\begin{proof}
We will prove this by induction. Lemma \ref{lem:correctness:base_case} proved the base case where $n=1$. One can see that the algorithm adheres to the base case in lines 5-7. Now, assume for the inductive step that if there exists a sweep-cover of any size $ < n$ on any $\mathcal{T}$, or any subtree on $\mathcal{T}$, then the algorithm is able to find it. Consider Lemma ~\ref{lem:all_sweep_covers} which shows that all sweep covers can be found by applying Lemma ~\ref{lem:singleton} and Lemma \ref{lem:swap_children}. Therefore, if the algorithm is to find all possible sweep covers of size $n$, it must apply Lemma ~\ref{lem:singleton} to all possible partitions of $C$. Ff a partition contains a singleton, it can be assumed a recursive call on that subtree will find all sweep covers of size $< n$ on that given subtree. One can see by lines 13-23 the algorithm achieves Lemma ~\ref{lem:singleton} and Lemma \ref{lem:swap_children} by assuming a recursive call returns sweep covers for a given size $< n$. Lines 24-25 show that if a given potential sweep cover is not of size $n$, then do not add it to $\mathcal{Q}$. If none are of size $n$, then $\mathcal{Q}$ is returned empty. Therefore, it is only possible to return all sweep covers of size $n$ or an empty set.  This shows the algorithm correctly finds all possible sweep covers for $n$, assuming the algorithm can find all sweep covers for $1 \rightarrow n - 1$.

%If we assume that the algorithm works for sweep covers of size $< n$ then by Lemma ~\ref{lem:all_sweep_covers} we have shown it works for all $n$ if the sweep-cover exists. 

%We will prove this is the case. One can see line 9 considers all possible partitions of $c$. The upper bound on the size of the partition is the minimum of n or $|c|$ because it is impossible to exceed $|c|$ partitions of a set of that size and if $n < |c|$ then any partition with $>n$ parts cannot be a sweep-cover of size $n$. One can see that we consider every possible partition of $c$ within these boundaries. We know by Lemma ~\ref{cor:partitions} that if R is a complete partition of c which contains $n$ parts then it can be considered a sweep-cover so we append it to the result, $\mathcal{Q}$. For lines 15-26 we can see 



%We have shown by Lemma \ref{lem:all_sweep_covers} that we can find all sweep covers by considering all partitions of $c$ and all ways of creating a sweep-cover by sweep covers of smaller sizes on subtrees rooted by nodes in $c$. One can see that lines 9-24 are a direct application of Lemma \ref{lem:singleton} and Corollary \ref{cor:partitions}. Also, if a Sweep 

%We want to consider all ways of partitioning these nodes because sets of siblings are the only possible sets within a sweep-cover. Therefore, we find all possible subsets of $c$. However, it is impossible to partition $c$ into more sets than there are nodes in $c$. Also, consider a collection of $n + 1$ disjoint subsets of $c$. Even if this forms a sweep-cover, it is too many sets for the sweep-cover of size $n$. Therefore, we only consider partitioning $c$ into 1 to the minimum of $|c|$ or $n$ so that both conditions are satisfied.

%By subdefinition \ref{sweep_cover:sibling}, all nodes within a set must be siblings. Therefore, we consider all possible ways of partitioning the nodes in $c$ into all sizes from 1 to $\min\{|c|,n+1\}$ parts.

%\input{Diagrams/children_lemma1.tex}


\end{proof}



==> Text/trash_text.tex <==


It is a well known fact that if a function is log-convex, then the product of the function over any integer partition is convex.

\begin{theorem}
Consider a positive, discrete, log-convex function $f(n)$ over $\mathbb{Z}_+$, i.e.,
\begin{align} 
    &\forall n \in \mathbb{Z}^+ : f(n-2)f(n) > f(n-1)^2 \label{eq:thm:log_convexity}
\end{align}

 Let $u(n)$ and $l(n)$ be the asymptotic upper bound and lower bound, respectively, of $f(n)$ such that $f(n) = O(u(n)) = \Omega(l(n))$. Define $g(n,m)$ to be a summation of the products of $f$ over integer compositions of $n$ into $m$ parts. 

\begin{equation}
    g(n,m) = \sum_{X \in \Gamma_{n,m} }{(\prod_{x_j \in X}f(x_j))} 
\end{equation}
Then, $g(n,m) = O\left({n - 1 \choose m - 1} u(n-1)u(1)^{m-1}\right) = \Omega\left({n - 1 \choose m - 1} l\left(\floor{\frac{n}{m}} + 1\right)^{n \mod m} l\left(\floor{\frac{n}{m}}\right)^{m - n \mod m} \right) $.
\label{thm:int_comp_convex_func}
\end{theorem}
We will prove Theorem \ref{thm:int_comp_convex_func} using the following proofs.

\begin{corollary}
Consider the log-convex function $f(n)$ over an ordered domain $\mathcal{C} \subseteq \mathbb{Z}_+$. Then, by induction, the following relationship holds,

\begin{align}
   \forall n \in \mathcal{C} :  \frac{f(n)}{f(n-1)} > \frac{f(n-1)}{f(n-2)} > \ldots > \frac{f(\mu)}{f(\mu - 1)},
\end{align}

where $\mu - 1$ is the infimum of $\mathcal{C}$. \label{cor:log_convex_ratio}
\end{corollary}



\begin{lemma}
Consider an integer composition $X \in \Gamma_{n,m}$ in the set of all integer compositions of $n$ into $m$ parts. Then, choose two parts in $x_j, x_v \in X$ such that $x_j \geq x_v$ and $x_v > 1$. Construct a new integer composition $Y \in \Gamma_{n,m}$ such that $\forall k \in \{ 1,...,m \} \backslash \{ j,v\}, x_k = y_k$. Let $y_j = x_j + 1$ and $y_v = x_v - 1$. Then,

\begin{align}
    \prod_{x_k \in X}f(x_k) < \prod_{y_k \in Y}f(y_k). \label{eq:lem:log_convex_max_incr1}
\end{align}
\label{lem:log_convex_max}

\end{lemma}
\begin{proof}
Note that by definition of $Y$,

\begin{align}
    \prod_{\forall k \in \{ 1,...,m \} \backslash \{ j,v\}}f(x_k) = \prod_{\forall k \in \{ 1,...,m \} \backslash \{ j,v\}}f(y_k). \label{eq:lem:log_convex_max_incr2}
\end{align}

 By dividing both sides in (\ref{eq:lem:log_convex_max_incr1}) by (\ref{eq:lem:log_convex_max_incr2}) and substituting in $y_j = x_j + 1$ and $y_v = x_v - 1$, we obtain

 
\begin{align}
    f(x_j)f(x_v) < f(x_j+1)f(x_v-1). \nonumber
\end{align}

Which implies,

\begin{align}
    \frac{f(x_v)}{f(x_v-1)} < \frac{f(x_j+1)}{f(x_j)}. \label{eq:lem:log_convex_max_incr3}
\end{align}
Corollary \ref{cor:log_convex_ratio} implies  (\ref{eq:lem:log_convex_max_incr3})
is always true because $x_j + 1 > x_v$.
\end{proof}

\begin{lemma}
By an extension of Lemma \ref{lem:log_convex_max}, the integer composition $X^* \in \Gamma_{n,m}$ that maximizes the product $\prod_{x_k \in X}f(x_k)$ is any permutation of $X^* = \{n - m + 1, 1, \ldots, 1  \}$. \label{lem:log_convex_max_vector}
\end{lemma}

\begin{proof}
 Begin with any integer composition $X \in \Gamma_{n,i}$ such that $X \ne X^*$. By consecutively applying Lemma \ref{lem:log_convex_max} to the integer composition $X$, the integer composition will converge to an integer composition $X'$ where one part $x'_k = n - m + 1$ and all other parts equal $1$. This integer composition has the same product at $X^*$ and is a permutation of $X^*$. 
\end{proof}

\begin{lemma}
By an extension of Lemma \ref{lem:log_convex_max_vector}, the integer composition $\bar{X} \in \Gamma_{n,m}$ that minimizes the product $\prod_{x_k \in \bar{X}}f(x_k)$ is any permutation of $\bar{X} = \{ \floor{\frac{n}{m}} + b_1, \floor{\frac{n}{m}} + b_2,  \ldots, \floor{\frac{n}{i}} + b_m \}$, where $b_k \in \{0,1\}$ such that $\sum_{k \leq i}b_k < m$.
\end{lemma}
\begin{proof}
 Consider any integer composition $X$ and apply the inverse of Lemma \ref{lem:log_convex_max} repeatedly to reduce the product $\prod_{x_k \in \bar{X}}f(x_k)$. In other words, construct a new integer composition $X'$ from $X$ by taking two parts, $x_j, x_v \in X$ such that $x_j > x_v$. Then, $x'_j = x_j - 1$ and $x'_v = x_v + 1$. Doing this will repeatedly will eventually construct an integer composition which is a permutation of $X$ and has the same product as $X$.
\end{proof}

\begin{lemma}
Consider a positive, discrete, log-convex function $f(n)$ over $\mathbb{Z}^+$. Let $u(n)$ be the asymptotic upper bound of $f(n)$ such that $f(n) = O(u(n))$. Define $g(n,m)$ to be a summation of the products of $f$ over integer compositions of $n$ into $m$ parts. Then, $g(n,m) = O\left( {n - 1 \choose m - 1} u(n-1)u(1)^{m-1}\right)$. \label{lem:convex_func_ub}
\end{lemma}
\begin{proof}
 By Lemma \ref{lem:log_convex_max_vector}, an integer composition $X$ that maximizes the product $\prod_{x_k \in X}f(x_k)$ is any permutation of $X^* = \left\{n - m + 1, 1, \ldots, 1  \right\}$. By replacing all terms in the summation with $X = X^*$, we have 
 \begin{align}
     g(n,m) < {n - 1 \choose m - 1} \prod_{x^*_k \in X^*}f(x^*_k) = {n - 1 \choose m - 1} f(n-m + 1)f(1)^{m-1}
 \end{align}
\end{proof}

\begin{lemma}
Consider a positive, discrete, log-convex function $f(n)$ over $\mathbb{Z}_+$. Let $l(n)$ be the asymptotic lower bound of $f(n)$ such that $f(n) = \Omega(l(n))$. Define $g(n,m)$ to be a summation of the products of $f$ over integer compositions of $n$ into $i$ parts. Then, $g(n,m) = \Omega\left({n - 1 \choose m - 1} l(\floor{\frac{n}{m}} + 1)^{n \text{ mod } m} l(\floor{\frac{n}{m}})^{m - n \text{ mod } m} \right)$. \label{lem:convex_func_lb}
\end{lemma}
\begin{proof}
 By Lemma \ref{lem:log_convex_max_vector}, an integer composition $X$ that minimizes the product $\prod_{x_k \in \bar{X}}f(x_k)$ is any permutation of $\bar{X} = \left\{ \floor{\frac{n}{m}} + b_1, \floor{\frac{n}{m}} + b_2,  \ldots, \floor{\frac{n}{m}} + b_i \right\}$, where $b_k \in \{0,1\}$ such that $\sum_{k \leq m}b_k < m$. By replacing all terms in the summation with $X = X^*$, we have 
 \begin{align}
     g(n,m) > {n - 1 \choose m - 1} \prod_{\bar{x}_k \in \bar{X}}f(\bar{x}_k) = {n - 1 \choose m - 1} f\left(\floor{\frac{n}{m}} + 1\right)^{(n \text{ mod } m)} f\left(\floor{\frac{n}{m}}\right)^{m - (n \text{ mod } m)}.
 \end{align}
\end{proof}

Theorem \ref{thm:int_comp_convex_func} holds due to Lemmas \ref{lem:convex_func_ub} and \ref{lem:convex_func_lb}.

However, for what conditions can $f(x)$ not be log-convex and the product still be log-convex? Namely, consider the following weaker conditions,

\begin{align}
    f(1) \geq 1 \label{eq:finite_difference}\\
    \frac{f(n)}{f(n-1)} > m \geq 2 \label{eq:const_ratio}.
\end{align}

\begin{corollary}
\begin{align}
  f(n) - f(n - 1) > f(n-1) - f(n - 2) : \forall n > 2
\end{align}
\end{corollary}
\begin{proof}
Note that this condition is equivalent to,

\begin{align}
  f(n)  > 2f(n-1) - f(n - 2) : \forall n > 2,
\end{align}
which is satisfied by $f(n)  > m f(n-1)$ if $m \geq 2$.
\end{proof}

\begin{corollary}
\begin{align}
  f(n) - f(n - 1) > n - 1 : \forall n \geq 2
\end{align}
\end{corollary}
\begin{proof}
By applying (\ref{eq:finite_difference})

\begin{align}
  f(n) - f(n - 1) > f(n-1) - f(n - 2) > ... > f(2) - f(1) > 1 : \forall n \geq 2,
\end{align}
which implies 

\begin{align}
  f(n) - f(n - 1) > n - 1 : \forall n \geq 2.
\end{align}
\end{proof}

We argue that if a function $f(n)$ satisfies both of these conditions, then the summation over the products of integer compositions is log-convex, even though $f(n)$ is not necessarily log-convex.

If $\frac{g(n,i)}{g(n-1,i)} = \omega(n)$, then $g(n,i)$ is log-convex. By a counting argument, we can rewrite the ratio between $g(n,i) $ and $g(n-1,i)$ as

\begin{align}
    \frac{g(n,i)}{g(n-1,i)} > \frac{{n - 2 \choose i - 1} \Tilde{g}(n,i) \frac{n - 1}{n - i + 1} }{{n - 2 \choose i - 1}}
\end{align}

where $\Tilde{g}(n,i)$ is the averaged difference between $g(n,i) $ and $g(n-1,i)$ per integer composition,

\begin{align}
    \Tilde{g}(n,i) = \frac{\sum_{X \in \mathcal{O}^{n - 1}_i} (f(x_{j+1}) - f(x_j))\prod_{x_l \not \in X \backslash x_j}f(x_l)}{{n - 2 \choose i - 1}} \label{eq:g_tilde}
\end{align}

Intuitively, we are summing up all the differences between $g(n,i) $ and $g(n-1,i)$ and averaging them into one ratio. By a counting argument, the number of terms in the summation in (\ref{eq:g_tilde}) is equal to ${n - 2 \choose i - 1}$. So, if every term in the summation is greater than $n - i$, then $\Tilde{g}(n,i) > n - i$. To show this, we use the conditions (\ref{eq:finite_difference}) and (\ref{eq:const_ratio}) on $f(n)$. 

Namely, we know by applying (\ref{eq:finite_difference}) that $f(x_{j+1}) - f(x_j) = f(n - \sum{x_l}) - f(n - \sum{x_l} - 1) > n - \sum{x_l}$. So,  Likewise, by inductively applying (\ref{eq:const_ratio}), we know that $f(x_j) > m^{x_j - 1}f(1)$. Substituting these relations into (\ref{eq:g_tilde}) gives us, 

\begin{align}
    (f(x_{j+1}) - f(x_j))\prod_{x_l \not \in X \backslash x_j}f(x_l) > (n - \sum{x_l}) m^{\sum{x_l} - i}f(1)^{i - 1}.
\end{align}

Then, the following relationship holds for every $ i < \sum{x_l} < n$, and therefore every $ 1 < x_j \leq n - i + 1$


\begin{align}
    (n - \sum{x_l}) f(1)^{i - 1} > \frac{n - i + 1}{m^{\sum{x_l} - i}}.
\end{align}



